Path placement optimization of manipulators based on energy consumption: application to the orthoglide 3-axis

This paper deals with the optimal path placement for a manipulator based on energy consumption. It proposes a methodology to determine the optimal location of a given test path within the workspace of a manipulator with minimal electric energy used by the actuators while taking into account the geometric, kinematic and dynamic constraints. The proposed methodology is applied to the Orthoglide~3-axis, a three-degree-of-freedom translational parallel kinematic machine (PKM), as an illustrative example.

==> 02D_Algorithm_PathPlacementOptimizationProblem_Detailed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resolution of the Path Placement Optimization Problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To solve the problem, a general optimization approach is proposed and illustrated in Fig.~\ref{fig:Flowchart}. The process can be classified in three major steps:
\begin{enumerate}
	\item 
%\begin{itemize}
%	\item
	Input Data:
	Manipulator geometric, dynamic and electric parameters along with the defintion of the required path are used as the known input data of the optimization problem. Base frame ${\cal F}_b$ and path frame ${\cal F}_p$ are respectively defined corresponding to the manipulator and the path geometry. Varaibles describing the location of ${\cal F}_p$ with respect to ${\cal F}_b$ will be the optimization decision variables. These parameters once defined remain out of the main optimization loop.
	\item
	Objective Function Evaluation: At this stage, manipulator synthesis is performed using its geometric, kinematic and dynamic models. Objective function and constraints are evaluated corresponding to the location of ${\cal F}_p$.
	\item
	Optimization algorithm: Objective fucntion and constraints evaluated previously are analyzed by means of the optimization algorithms. Once the constraints are satisfied, objective function is tested for its optimum value. Convergence cretia are verified and hence a decision is made to continue or teminate the optimization loop iterations depending on the optimization routine in use.
	\end{enumerate}
Finally, the optimum path placement is obatined by means of the position of point $O_p(x_{O_p}^*,~y_{O_p}^*,~z_{O_p}^*)$ and the orientation of ${\cal F}_p$ with respect to ${\cal F}_b$, defined by $(\phi^*,~\theta^*,~\psi^* )$.
%%%%%%%%%%%%%%%======================================================================================
To solve the problem, a general optimization approach is proposed and illustrated by means of Fig.~\ref{fig:Flowchart}:
\begin{enumerate}
	\item 
%\begin{itemize}
%	\item
	Definition of the base reference frame ${\cal F}_b$;
	\item
 	definition of the path reference frame ${\cal F}_p$ at a suitable reference point of the path;
	\item
 	complete description of the given path in ${\cal F}_p$. At this stage, path, velocity and acceleration profiles of end-effector are defined in ${\cal F}_p$;
	\item
 	with an initial guess of design variables
 	$\mathbf{x}_0=[x_{{O_p}_0} \quad y_{{O_p}_0} \quad z_{{O_p}_0} \quad \phi_{_0} \quad \theta_{_0} \quad \psi_{_0}]^T$,
 	 ${\cal F}_p$ is located with respect to ${\cal F}_b$;
 	 	\item
 	the transformation matrix $\mathbf{^\textit{b}T_\textit{p}}$ is calculated from $\mathbf{x}$;
 	 	\item
 	using $\mathbf{^\textit{b}T_\textit{p}}$, trajectory parameters are calculated in ${\cal F}_b$, i.e., calculation of the Cartesian velocities and accelerations of the end-effector;
 	 	\item
 	the actuated variables $q_i$ are calculated by means of the Inverse Geometric Model (IGM) of the manipulator;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\begin{figure}[tbp]
  \centering
  \psfrag{A}[c][c][1][0.8]{\textcolor{myblue}{Input Data}}
  \psfrag{A11}[c][c][1][0.8]{Geometric \& Dynamic Parameters}
  \psfrag{A12}[c][c][1][0.8]{Definition of base frame ${\cal F}_b$}
  \psfrag{A13}[c][c][1][0.8]{Electric motors parameters}
  \psfrag{A14}[c][c][1][0.8]{Path definition}
  \psfrag{A2}[c][c][1][0.8]{Definition of Path frame ${\cal F}_p$}
  \psfrag{A3}[c][c][1][0.8]{Trajectory Definition in ${\cal F}_p$}
  \psfrag{A4}[c][c][1][0.8]{Initial Guess $\mathbf{x}_0$}
  \psfrag{A41}[c][c][0.8]{$\mathbf{x}_{_0}=[x_{{Op}_0} \quad y_{{Op}_0} \quad z_{{Op}_0} \quad \phi_{_0} \quad \theta_{_0} \quad \psi_{_0} ]^T$}

  \psfrag{B}[c][c][1][0.8]{\textcolor{myblue}{Objective Function}}
  \psfrag{BB}[c][c][1][0.8]{\textcolor{myblue}{Computation}}
  \psfrag{B1}[c][c][1][0.8]{Transformation Matrix $\mathbf{^\textit{b}T_\textit{p}}$}
  \psfrag{B2}[c][c][1][0.8]{Trajectory Definition in ${\cal F}_b$}
  \psfrag{B31}[c][c][1][0.8]{Inverse Geometric Model}
  \psfrag{B32}[c][c][1][0.8]{Inverse Kinematic Model}
  \psfrag{B33}[c][c][1][0.8]{Inverse Dynamic Model}
  \psfrag{B4}[c][c][1][0.8]{Objective and Constraints Evaluation}
  
  \psfrag{C}[c][c][1]{\textcolor{myblue}{Optimization Algorithm}}
  \psfrag{C1}[c][c][0.8]{$q_{lb}\leq q_i\leq q_{ub}$}
  \psfrag{C12}[c][c][0.8]{$\dot{q}_i\leq \dot{q}_{ub}$}
  \psfrag{C13}[c][c][0.8]{$\tau_i\leq \tau_{ub}$}
  
  \psfrag{C2}[c][c][1]{$E_t=E_{min}$}
  \psfrag{C3}[c][c][1]{$\mathbf{x}_j=\mathbf{x}_{j+1}$}
  
  \psfrag{D1}[c][c][1]{Optimum value}
  \psfrag{D2}[c][c][1]{$\mathbf{x}^*=\mathbf{x}_j$}
  
  \psfrag{Y1}[c][c][1][0.8]{Yes}
  \psfrag{Y2}[c][c][1][0.8]{Yes}
  \psfrag{N1}[c][c][1][0.8]{No}
  \psfrag{N2}[c][c][1][0.8]{No}

	\includegraphics[width=14cm]{Fig2_Flowchart}
  \caption{Flowchart of path placement optimization process}
  \label{fig:Flowchart}
	\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	 	\item
 	the actuators velocity $\dot{q}_i$ and acceleration $\ddot{q}_i$ profiles are derived from the Inverse kinematic Model (IKM) of the manipulator; 
 	 	\item
 	the actuators torques $\tau_i$ are derived from the Inverse dynamic model (IDM) of the manipulator;
 	 	\item
 	the current $I$ and voltage $V_e$ required by each actuator are calculated by using the actuators torques, velocities, the motors torque sensitivity factor $K_t$ and the back electromotive force constant $K_e$, as defined in Eqs.(\ref{Eq:i}) and (\ref{Eq:Ve});
 	 	\item
 	the electric power $P_{T_i}$ consumed by the $i^{th}$ actuator is obtained from the current, voltage and actuators electric constants, as defined in Eq. (\ref{Eq:Pe});
 	 	\item
 	the electric energy $E_i$ consumed by the $i^{th}$ actuator is then calculated by integrating the consumed power $P_{Ti}$ over total trajectory time $T$, as given by Eq. (\ref{Eq:E}). Subsequently, the total electric energy $E_t$ used by the manipulator is obtained by adding up the energy consumed by all actuators;
 	 	\item
 	the constraints and the convergence criteria are verified at each iteration $j$. The convergence criteria are upto the user. They can be the constraints, objective function tolerances, the number of iterations and so on;
 	 	\item
 	the optimization algorithm (iterative process) is used to find out the optimum design variables, namely, $\mathbf{x}^*$=[$x_{O_p}^* \quad y_{O_p}^* \quad  z_{O_p}^* \quad   \phi^* \quad   \theta^* \quad  \psi^* $]$^T$  in order to minimize $E$.
\end{enumerate}
Finally, the optimum path placement is obatined by means of the position of point $O_p(x_{O_p}^*,~y_{O_p}^*,~z_{O_p}^*)$ and the orientation of ${\cal F}_p$ with respect to ${\cal F}_b$, defined by $(\phi^*,~\theta^*,~\psi^* )$.
%%\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> macros.tex <==
% All Multi-line comments appear at the BEGININING of a macro.
% "Note"s, appear at the BOTTOM of a macro or set of macros.
% Some macros have wide application. Do not let comments narrow their scope.
% The comments are only for a short reference or for beginners.
% Refer to any LaTeX guide for details.


%\newcommand{\BIBand}{and}

\newcommand{\gbf}[1] {\mbox{\boldmath${#1}$\unboldmath}}% inserts 'g'reek 'b'old 'f'ace symbols eg. \gbf{\alpha} in text.
\newcommand{\be}{\begin{equation}}%starts equation environment with equation numbers
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}%starts equation environment with equation numbers
\newcommand{\eeq}{\end{equation}}
\newcommand{\bed}{\begin{displaymath}}%starts equation environment without equation numbers
\newcommand{\eed}{\end{displaymath}}

% array of equations. If equations are separated by \\ each equation is numbered,
% else if they are separated by \cr the whole set is given a single equation number.
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

% 'a'rray of equations, with 'n'o equation 'n'umbers
\newcommand{\beqann}{\begin{eqnarray*}}
\newcommand{\eeqann}{\end{eqnarray*}}

%Note. For an array of equations to appear the above two environments may be used.
% In order to align all equations at '=' sign, enter the equation as having three columns
% with '=' in the centre column, using the '&' column seperator. This is easy to implement. eg.
%
%\beqa
%\M(\q)\qdd+\vv(\q,\qd)&=&{\E}(\q)\uv \cr
%\C(\q)&=&\bf 0
%\eeqa
%
% This should print the two equations aligned at '=' signs.
% end NOTE
%
% Place equation arrays within \bseq and \eseq to number subequations.
\newcommand{\bseq}{\begin{subequations}}
\newcommand{\eseq}{\end{subequations}}
% example  \bseq \beqa a&=&b \\ c&=&d \\ e&=&f \eeqa \eseq
% This will     1. align the three equations at = sign (&=& column separater)
%       2. give each equation a number (\\ equation separator)
%       3. give each equation a subequation number (\bseq and \eseq)
% Note. you need to have the equations.sty package
% add to preamble: \usepackage{equations}
% end Note

\newcommand{\case}[1]{ \left\{ \begin{array}{ll} #1 \end{array} \right. }
\newcommand{\dx}{\dot x} %scalar dx/dt
\newcommand{\ddx}{\ddot x} %scalar d2x/dt2
\newcommand{\dy}{\dot y} %scalar dy/dt
\newcommand{\ddy}{\ddot y} %scalar d2y/dt2
\newcommand{\dz}{\dot z} %scalar dz/dt
\newcommand{\ddz}{\ddot z} %scalar d2z/dt2
\newcommand{\om}{\omega}
\newcommand{\omn}{\omega_n}
\newcommand{\omd}{\omega_d}
\newcommand{\mat}[2]{\left[ \begin{array}{#1} #2 \end{array} \right] } %can use smatrix instead
\newcommand{\ora}[1]{\overrightarrow{#1}} %'o'verhead 'r'ight pointing 'a'rrow, on the argument
\newcommand{\smatrix}[1]{\left[\matrix{#1}\right]}%'s'quare bracketed 'matrix'. eg. smatrix{a& b\cr c& d} will produce a square bracketed matrix with elements a,b;c,d.
\newcommand{\smatrixams}[1]{\left[\begin{matrix} #1 \end{matrix}\right]}%amspackage compliant
\newcommand{\Smatrix}[2]{\left[\ba{#1}#2\ea\right]}% same as \mat command.
% begins an array. eg. \ba{lr} a&b\\c&d \ea, will produce a 2x2 array with elements a,b;c,d.
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bdq}{{\bf \dot{q}}}% boldface dot_q
\newcommand{\bq}{{\bf q}}% boldface q

%Note. All Macros in the above set must be used in an equation environment (or b/w $...$)

% creates a boxed equation. The first argument is the width of box while the second argument is the equation itself. eg. \boxedeq{3cm}{i+1=3} will create a numbered equation in a box of 3cm width.
\newcommand{\boxedeq}[2]{
    \vspace*{0.2cm}
    \begin{center}
    \fbox{
        \parbox{#1}{
            \begin{equation}
            #2
            \end{equation}
        }
    }
    \end{center}
    \vspace*{0.2cm}
}

% creates an array of boxed equations. The first argument is the width of box while the second argument is the equation itself. eg. \boxedea{3cm}{i+1=3\\i+3=5} will create two numbered equations in a box of 3cm width, the height adjusted automatically.
\newcommand{\boxedeqa}[2]{
    \vspace*{0.2cm}
    \begin{center}
    \fbox{
        \parbox{#1}{
            \begin{eqnarray}
            #2
            \end{eqnarray}
        }
    }
    \end{center}
    \vspace*{0.2cm}
}

%inserts a figure. Must put "\usepackage{epsfig}" between documentclass and begin{document}
% eg. \figureinsert{<filename>}{<width>}{<caption>}{<label>}, where <label> is a reference to this figure.
\newcommand{\figureinsert}[4]{
\begin{figure}[htbp]
\begin{center}
\mbox{\psfig{figure=#1,width=#2}}
\parbox{11cm}{\caption{#3} \label{#4}}
\end{center}
\end{figure}
}

\newcommand{\yzi}{y_{\scriptscriptstyle ZI}}
\newcommand{\yzs}{y_{\scriptscriptstyle ZS}}

\newcommand{\of}{\overline f} %f_bar. Must be issued in equation environment.
\newcommand{\dw}{\dot w} %w_dot. Must be issued in equation environment.
\newcommand{\ddw}{\ddot w} %w_double dot. Must be issued in equation environment.
\newcommand{\dv}{\dot v} %v_dot. Must be issued in equation environment.
\newcommand{\ddv}{\ddot v} %v_double dot. Must be issued in equation environment.

%Matrices and vectors.
%Rule followed. 1. All Matrices boldface capitals, 2. All vectors boldface small.
\newcommand{\A}{{\bf A}} %bold face A, used for matrices
\newcommand{\Am}{{\bf A}}
\newcommand{\av}{{\bf a}} % added jan12, 2002 %constraint vector c
\newcommand{\avh}{{\hat{\av}}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\B}{{\bf B}}
\newcommand{\Bd}{\dot{\B}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bv}{{\bf b}}
\newcommand{\bvh}{\hat{\bv}}
\newcommand{\bvb}{\bar{\bv}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\C}{{\bf C}}
\newcommand{\cv}{{\bf c}} % added jan12, 2002 %constraint vector c
\newcommand{\cvh}{\hat{\cv}}
\newcommand{\D}{{\bf D}}
\newcommand{\dvv}{{\bf d}} %added jul30, 2002
\newcommand{\ev}{{\bf e}}
\newcommand{\E}{{\bf E}}
\newcommand{\Em}{{\bf E}}
\newcommand{\F}{{\bf F}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\f}{{\bf f}}
\newcommand{\fv}{{\bf f}}
\newcommand{\G}{{\bf G}}
\newcommand{\gv}{{\bf g}} %added jul30, 2002 for all vectors. This makes thing consistent. Old ones are kept for compatibility.
\newcommand{\g}{{\bf g}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\hv}{{\bf h}} %added jul30, 2002
\newcommand{\h}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\I}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\K}{{\bf K}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\mv}{{\bf m}}
\newcommand{\M}{{\bf M}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\N}{{\bf N}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\nv}{{\bf n}}
\newcommand{\Pm}{{\bf P}} % since \P is reserved, \Pm is used for matrix P.
\newcommand{\p}{{\bf p}}  % added june12, 2002
\newcommand{\pv}{{\bf p}} %added jul30, 2002
\newcommand{\pvd}{\dot{\pv}}
\newcommand{\tildepv}{{\tilde{\pv}}}
\newcommand{\Q}{{\bf Q}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\qv}{{\bf q}} %added jul30, 2002
\newcommand{\q}{{\bf q}}
\newcommand{\qd}{{\dot \q}}
\newcommand{\qdd}{{\ddot \q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\R}{{\bf R}}
\newcommand{\rv}{{\bf r}} %added jul30, 2002
\newcommand{\br}{{\bf r}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\sv}{{\bf s}}
\newcommand{\T}{{\bf T}}
\newcommand{\Tm}{{\bf T}} %added for streamlined entries
\newcommand{\tv}{{\bf t}} %vector t, since \t is reserved
\newcommand{\tvd}{\dot{\tv}}
\newcommand{\Um}{{\bf U}}
\newcommand{\uv}{{\bf u}} %vector u, since \u is reserved
\newcommand{\ud}{{\dot \uv}}
\newcommand{\udd}{{\ddot \u}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\vv}{{\bf v}} %vector v, since \v is reserved
\newcommand{\vd}{{\dot \vv}}
\newcommand{\W}{{\bf W}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\wv}{{\bf w}} %added jul30, 2002
\newcommand{\w}{{\bf w}}
\newcommand{\wdv}{{\dot \w}}
\newcommand{\xv}{{\bf x}} %added jul30, 2002
\newcommand{\x}{{\bf x}}
\newcommand{\xd}{\dot \x} %vector dx/dt
\newcommand{\xdd}{\ddot \x} %vector d2x/dt2
\newcommand{\yv}{{\bf y}} %added jul30, 2002
\newcommand{\y}{{\bf y}}
\newcommand{\yd}{\dot \y}
\newcommand{\ydd}{\ddot \y}
\newcommand{\zv}{{\bf z}} %added jul30, 2002
\newcommand{\z}{{\bf z}}
\newcommand{\zd}{\dot \z}
\newcommand{\zdd}{\ddot \z}

\newcommand{\Om}{{\bf\Omega}}
\newcommand{\Omm}{{\bf O}}
\newcommand{\0}{{\bf 0}}
\newcommand{\1}{{\bf 1}}



\newcommand{\ctn}[1]{\cos[k\omega_0(t_0+\frac{#1 T}{N})]}% must be in equation environment
\newcommand{\stn}[1]{\sin[k\omega_0(t_0+\frac{#1 T}{N})]}% must be in equation environment eg. $\stn{5}$

\newcommand{\negr}[1]{{\bf {#1}}}
\newcommand{\nigr}[2]{{\bf {#1}}_{#2}}
\newcommand{\negrg}[1]{{\gbf {#1}}}
\newcommand{\nigrg}[2]{{\gbf {#1}}_{#2}}
\newcommand{\thE}{\theta_E}

\newcommand{\nind}{\noindent}
\newcommand{\oom}{{\overline\omega}}% omega_bar
\newcommand{\on}{{\overline\nu}}%nu_bar
\newcommand{\dxi}{{\dot\xi}}
\newcommand{\oc}{{\overline c}}% c_bar
\newcommand{\os}{{\overline s}}% s_bar

\newcommand{\bfTheta}{\gbf{\Theta}} %boldface Capital Theta.
\newcommand{\dtheta}{{\dot\theta}}
\newcommand{\ddtheta}{{\ddot\theta}}
\newcommand{\dphi}{{\dot\phi}}
\newcommand{\ddphi}{{\ddot\phi}}
\newcommand{\dalpha}{{\dot\alpha}} %added jan11,2002
\newcommand{\ddalpha}{{\ddot\alpha}}%added jan11,2002
\newcommand{\dnu}{{\dot\nu}} % added jan12, 2002
\newcommand{\ddnu}{{\ddot\nu}} % added jan12, 2002
\newcommand{\dupsilon}{{\dot\upsilon}} % added jan12, 2002
\newcommand{\ddupsilon}{{\ddot\upsilon}} % added jan12, 2002
\newcommand{\taubar}{{\bar{\gbf{\tau}}}}
\newcommand{\tautilde}{{\tilde{\gbf{\tau}}}}


\newcommand{\ol}[1]{\overline{\mbox{${#1}$}}}

\newcommand{\partder}[2]{\frac{\partial{#1}}{\partial{#2}}} %'par'tial 'der'ivative eg. \partder{y}{x}
\newcommand{\secpartder}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}} %second partial derivative.
\newcommand{\secpartdermix}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}%second mixed partial derivate
\newcommand{\thipartder}[2]{\frac{\partial^3{#1}}{\partial{#2}^3}}%'thi'rd 'par'tial 'der'ivative
\newcommand{\foupartder}[2]{\frac{\partial^4{#1}}{\partial{#2}^4}}% 'fou'rth 'par'tial 'der'ivative

\def\oa{\overline{a}}%a_bar
\def\meanfreq{{\overline\omega}}
%\newtheorem{theorem}{Theorem}
%\newtheorem{example}{Example}[section]
%\newcommand{\eqref}[1]{{eq.(\ref{#1})}}


\newcommand{\Phim}{\gbf{\Phi}}
\newcommand{\Phimd}{\dot{\gbf{\Phi}}}


\newcommand{\dmatrix}[1]{\smatrix{#1^I&&\cr&[\ ]^{II}&\cr&&[\ ]^{III}}} % will produce matrix representing all three chains for three chains where #1 is of the form \smatrix{}
\newcommand{\dmatrixams}[1]{\smatrixams{#1^I&&\cr&[\ ]^{II}&\cr&&[\ ]^{III}}} % will produce matrix representing all three chains for three chains where #1 is of the form \smatrix{}
\newcommand{\needimprovement}{\footnote{Rem: text needs improvement}}

